Assessment of the Reliablity of a Model's Decision by Generalizing Attribution to the Wavelet Domain

Neural networks have shown remarkable performance in computer vision, but their deployment in numerous scientific and technical fields is challenging due to their black-box nature. Scientists and practitioners need to evaluate the reliability of a decision, i.e., to know simultaneously if a model relies on the relevant features and whether these features are robust to image corruptions. Existing attribution methods aim to provide human-understandable explanations by highlighting important regions in the image domain, but fail to fully characterize a decision process's reliability. To bridge this gap, we introduce the Wavelet sCale Attribution Method (WCAM), a generalization of attribution from the pixel domain to the space-scale domain using wavelet transforms. Attribution in the wavelet domain reveals where and on what scales the model focuses, thus enabling us to assess whether a decision is reliable. Our code is accessible here: \url{https://github.com/gabrielkasmi/spectral-attribution}.

==> content/comparison.tex <==
\paragraph{Models} The model testbench comprises convolutional neural networks (CNNs), embodied by the ResNet-50 \cite{he_deep_2016} model and the vision transformers, and more specifically, the ViT-B16 architecture, introduced by \cite{dosovitskiy_image_2021}. We consider six popular training strategies. Following \cite{chen_rethinking_2022}, we distinguish three training families: the "standard training" (ST) corresponding to the off-the-shelf use of a ResNet-50 trained on ImageNet, the "Robust training" (RT) approaches (AugMix \cite{hendrycks_augmix_2020}, PixMix \cite{hendrycks_pixmix_2022} and SIN \cite{geirhos_imagenet-trained_2023}), and the "adversarial training" (AT) (standard adversarial, \cite{madry_towards_2019}, the fast training approach  \cite{wong_fast_2020}, and the "free" method \cite{shafahi_adversarial_2019}). We implement robust and adversarial methods on a ResNet-50 backbone.

\paragraph{Datasets} We focus on ImageNet \cite{russakovsky_imagenet_2015} and ImageNet-C \cite{hendrycks_benchmarking_2019}. ImageNet-C features common image perturbations such as blur, pixelation, {\tt .jpeg} compression, and defocus blur that can occur in real life. Strengths levels, ranging from 1 to 6, can be applied to the perturbations. The higher the strength, the stronger the perturbation. When needed, we generate corrupted image samples using ImageNet-C source code. %In appendix \ref{sec:imagenet-e}, we apply the WCAM to other datasets and demonstrate its ability to troubleshoot a broader scope of distribution shifts ({\it e.g.}, renditions \cite{hendrycks_many_2021} and natural adversarial examples \cite{hendrycks_natural_2021}). We do not consider datasets such as CIFAR-\{10-100\} \cite{krizhevsky_learning_2009} or TinyImageNet \cite{le_tiny_2015} as the image size of these datasets is too small to decompose the image above one level meaningfully. 

% autres datasets, voir ceux qui sont été proposés


\subsection{Robustness of the model's predictions}

% Réinjecte les résultats obtenus en annexe: la WCAM permet de caractériser la robustesse des décisions d'un modèle
% Instance based evaluation : robustness vs/ RM par exemple ?

%seulement caractérisés en fréquence 
% objectif: retomber sur les résultats de travaux antérieurs

The scale embeddings introduced in section \ref{sec:methods-wcam} enable us to estimate the importance of each scale component into the final prediction. By definition of the wavelet transform, we have an equivalence between the scale levels in the wavelet domain and the frequency levels in the Fourier domain. The smallest scales correspond to the highest frequencies, and the largest scales (including those captured by the approximation coefficients) to the lowest frequencies. Therefore by ranking the entries of the scale embeddings as $z = (z_a, z_{1,v}, z_{1,d}, z_{1,h}, \dots, z_{L,v}, z_{L,d},z_{L,h})$ where $a$ corresponds to the approximation coefficients at $l\in\{1,\dots,L\}$ is the level, the scale embedding captures the importance of the frequency components by increasing order. In appendix \ref{sec:fourier-existing} we provide further empirical backing of the equivalence between Fourier and wavelet domains regarding the quantification of the frequency importance. 

We consider 100 images randomly sampled from the ImageNet validation set. We consider AT, RT and BT models, following the taxonomy of \cite{chen_rethinking_2022}. For each model and each image, we compute the WCAM and the associated scale embedding. We then average the embeddings for each model. For the AT and RT models, we average the average embeddings to compute a single embedding encompassing all models of these classes.

%\subsection{Highlighting the scale bias}

\subsection{Evaluating the scale consistency of the scale embeddings}

The scale embeddings represent the model's prediction in the scale space $\mathbb{R}^S$. By computing the distance between two embeddings, we measure their similarity in this space. If the distance between two embeddings is 0, it means that the model relied on the same scales to make its prediction. On the other hand, the larger the distance, the higher the discrepancy and thus the {\it inconsistency} between predictions. Formally, we can compute the distance $d(z_i, z_j)\equiv d_{i,j}$ between two scales embeddings $z_i$ and $z_j$ corresponding to two images $i$ and $j$ of a batch $B$ of images. The average distance $\bar{d}$ informs us about the scale consistency of the batch $B$. To measure the scale consistency, we evaluate a batch $B$ of $n$ images randomly sampled from ImageNet and class-specitic batches $B_1,\dots, B_c$ containing only images of the same class. We compute the average distance to evaluate the scale consistency. 







% mettre en avant le 

==> content/results.tex <==
%\subsection{Assessing the robustness of a classifier}

\paragraph{Robust models favor large scales} \autoref{fig:fcam-wcam-equivalence} presents the characterization of the robustness of a model. We can see that robust models favor large scales (i.e., low-frequencies) over small scales (i.e., high-frequencies). The WCAM enables for a characterization of robust models by estimating the importance of each frequency component in the final prediction. 

In \autoref{fig:approx} we consider all coefficient (including the approximation coefficients). As with a five level decomposition, the approximation coefficients still capture most of the content of the image, their importance is much larger than the importance of the detail coefficients. Therefore, in \autoref{fig:detail} we focus on the detail coefficients only. We can see that the ordering from the detail coefficients corresponding to the largest scales from those corresponding to the highest remains the same. These results are in line with existing works \cite{zhang_range_2022,chen_rethinking_2022,wang_high-frequency_2020,yin_fourier_2020} and show that the WCAM correctly estimates the robustness of a model.


\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/appendix/wcam-fcam-consistency-complete.pdf}
  \caption{Representation with all coefficients}
  \label{fig:approx}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/appendix/wcam-fcam-consistency-complete-no-approx.pdf}
  \caption{Representation with detail coefficients only}
  \label{fig:detail}
\end{subfigure}
\caption{Representation of the scales in the WCAM as frequencies. Levels (numbered 1 to 5) are ranked by descending order, from the coarser scales ({\it i.e.}, lowest frequencies) to the finest scales ({\it i.e.} highest frequencies). For a given level, labels "d", "h" "v" stand for the "diagonal", "horizontal" and "vertical" components. Computation of the importance for a given component is based on the sum of the Sobol indices for this components normalized by the total number of indices devoted to this scale. Computations are based on a 5-level dyadic decomposition of the input. "ST", "RT" and "AT" stand for "standard training", "robust training" and "adversarial training" respectively.}
    \label{fig:fcam-wcam-equivalence}
\end{figure}

%\paragraph{Class-wise robustness} Carrying out the same analysis, we can also evaluate the reliance on low or high frequency components across different classes. \autoref{} shows 
% Si le temps le permet, further discussion on the class wise robustness

% class wise robustness
% histogrammes pour différents modèles

\paragraph{Unveiling the scale inconsistency} \autoref{fig:edm_in} plots the average distance between two scale embeddings across 20 randomly sampled ImageNet classes. For each class, we compute the average distance between 50 scale embeddings. We can see that (i) the average difference varies among the classes and significantly differs from the noise attributable to randomness (bottom green dotted line). (ii) we can see that the distance between two random ImageNet images is not different from intra-class distances. We interpret this result as evidence from the fact that when shifting from one instance to the other, the model does not necessarily relies on the same scale, i.e. on the same factors to make its prediction. 

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.7\textwidth]{figs/edm_class_in-full_ci.pdf}
    \caption{Average distance in the scale domain between samples belonging to the same class. The noise line plots the background noise due to the sampling process. Continuous green lines plot the 95\% confidence interval around the average noise.}
    \label{fig:edm_in}
\end{figure}

\autoref{fig:scale_inconsistency} qualitatively illustrates the scale inconsistency for different models and different instances of the same class. We can see that models do not rely on the same factors. This suggests that the importance of features depends on the context and explains why image perturbations don't have a uniform effect on predictions. 

\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{figs/examples_scale_inconsistency.pdf}
    \caption{Example of scale inconsistencies for images of the same class (columns) for different models (rows : middle row: ResNet \cite{he_deep_2016}, bottom row : ViT \cite{dosovitskiy_image_2021}). The WCAM shows that depending of the image, the localization in the space-scale domain of the important factors differs, meaning that the model predicts the class according to different characteristics.}
    \label{fig:scale_inconsistency}
\end{figure}
% dans l'annexe, l'expérience des removal (avec le dataset suggéré par 1)

% 





%\autoref{} plots the WCAM for several models and several perturbations of the same image. All models (rows) correctly predict the image, no matter the perturbation (columns). However, we can see that the localization of the important factors greatly differs. Shifting from ERM (second row) to AugMix (second row), we can see that the important factors are more concentrated in the low frequencies region. However, no matter the model, we can see that the localization in scale of the important factor changes. 

% additional plots: appendix
\paragraph{Mechanisms} The scale inconsistency we uncover in the wavelet domain in a concurrent work \cite{wang_what_2023}. This work showed that learning shortcuts \cite{geirhos_shortcut_2020} can be characterized in the frequency domain: models tend to favor the most distinctive frequencies to make a prediction. These shortcuts in the Fourier domain are referred to as frequency shortcuts \cite{wang_frequency_2022}. Crucially, it also documents that these shortcuts are context dependent. Our results provide a more general characterization of this phenomenon, as it affects not only CNNs, but also transformers, and data augmentation techniques cannot mitigate it. Therefore, the reason behind these frequency shortcuts appears to be the optimization process. In that light, recent work \cite{pezeshki_gradient_2021} introduced the notion of {\it gradient starvation} phenomenon to explain learning shortcuts. According to this theory, "{\it when a feature is learned faster than the others, the gradient contribution of examples that contain this feature is diminished}."
